A Quasi-Newton Primal-Dual Algorithm with Line Search

Quasi-Newton methods refer to a class of algorithms at the interface between first and second order methods. They aim to progress as substantially as second order methods per iteration, while maintaining the computational complexity of first order methods. The approximation of second order information by first order derivatives can be expressed as adopting a variable metric, which for (limited memory) quasi-Newton methods is of type ``identity $\pm$ low rank''. This paper continues the effort to make these powerful methods available for non-smooth systems occurring, for example, in large scale Machine Learning applications by exploiting this special structure. We develop a line search variant of a recently introduced quasi-Newton primal-dual algorithm, which adds significant flexibility, admits larger steps per iteration, and circumvents the complicated precalculation of a certain operator norm. We prove convergence, including convergence rates, for our proposed method and outperform related algorithms in a large scale image deblurring application.

==> bfgs_sr1_metric.tex <==
\section{Computing and Representing the quasi-Newton Metric} \label{sec:bfgs-sr1-metric}

In this section, we abuse notation in order to follow the conventions of quasi-Newton methods\footnote{For example, the variable $y\iter\k$ defined in \eqref{eq:s-and-y} is not the dual variable in Algorithm~\ref{Alg:QN-PDHG-line}.}. The metric $M_k$ is expected to be an approximation of the Hessian $\nabla^2 h(x^k)$ at $x^k$ for the $k$-th iteration. The most popular quasi-Newton methods are the SR1 and BFGS methods (and their low-memory variants), which update $M_k$ by adding a rank-one modification (SR1 method)
\begin{equation}
    M_{k+1}:= M^{SR1}_{k+1}=M_k + \frac{ (y^k-M_ks^k)(y^k-M_ks^k)^\top }{ (y^k-M_ks^k)^\top s^k}\,,
\end{equation}
or a rank-two modification (BFGS method)
\begin{equation}
    M_{k+1}\coloneqq M^{BFGS}_{k+1}= M_k + \frac{y^k(y^k)^\top }{(s^k)^\top y^k } - \frac{M_ks^k(s^k)^\top M_k}{(s^k)^\top M_ks_k}\,,
\end{equation}
respectively, where
\begin{equation}\label{eq:s-and-y}
    s^k:=x^{k+1}-x^k\quad\text{and}\quad y^k := \nabla h(x^{k+1}) - \nabla h(x^k) \,.
\end{equation}
In order to apply quasi-Newton methods on large-scale problems, \emph{$m$-limited memory quasi-Newton methods} are adopted \cite{kanzow2022efficient}, with the most popular version being L-BFGS \cite{wright1999numerical}. It means that instead of generating $M_k$ via all previous $s^i$ and $y^i$ for $i=1,\ldots, k$ and $M_0$, for each $k$, the metric $M_k$ is re-computed based on $M_{k,0}$ and the most recent $m$ vectors $s^i$ and $y^i$ for $i=k-m+1,\ldots,k$, if $k\geq m$. Usually, $m$ is very small, such that only a small storage will be required. 
%Since for each iteration the update of  limited memory versions may not start with the same initial matrix $M_0$, we use the notation $M_{k,0}$ to stress the dependence on the $k$-th iterate.
As pointed out by \cite{byrd1994representations}, the matrices of the $m$-limited memory version of quasi-Newton methods have a compact representation of the form
\begin{equation}\label{eq:metric-compact}
    M_k=M_{k,0}+ A_kQ_k^{-1}A_k^\top \,,
\end{equation}
where $M_{k,0}\in\R^{n\times n}$, $n=\dim(X)$, is a symmetric positive definite matrix, $A_k\in \R^{n\times m}$, and a symmetric and non-singular matrix $Q_k\in\R^{m\times m}$ ($m\ll n$). 
For limited memory BFGS (known as L-BFGS), we have the following block-matrix representation
\begin{equation}
    A_k = \begin{bmatrix}M_{k,0}S_k&Y_k\end{bmatrix}\in \R^{n\times 2m}\quad\mathrm{and}\quad Q_k=\begin{bmatrix}
        -S_k^* M_{k,0}S_k&-L_k\\
        -L_k^* & D_k\\ 
    \end{bmatrix}\in \R^{2m\times 2m}\,,
\end{equation}
where $S_k$ and $Y_k$ are matrices collecting the $m$ most recent vectors in \eqref{eq:s-and-y} as columns, $D_k := D(S_k^\top Y_k)$ and $L_k :=L(S_k^\top Y_k)$ refer to the diagonal $D(\cdot)$ and the strict lower triangular $L(\cdot)$ part of the matrix $S_k^\top Y_k$, respectively. By using a spectral decomposition $Q^{-1}=V\Lambda V^\top $ with orthogonal $V\in \R^{s\times s}$ and diagonal $\Lambda\in\R^{s\times s}$, for some $s\in\N$, \eqref{eq:metric-compact} is transformed into the compact representation
\begin{equation}\label{metric}
    M_k = M_{k,0} + U_1U_1^\top  - U_2 U_2^\top \,,
\end{equation}
for some $U_1\in\R^{n\times m}$ and $U_2\in\R^{n\times m}$. In detail, since $\Lambda$ is a diagonal matrix with eigenvalues $\lambda_i$, $i=1,2,\ldots,s$ of $Q_k^{-1}$ on the diagonal, we decompose $\Lambda = \Lambda_1 -\Lambda_2$ where $\Lambda_1$, given by $(\Lambda_1)_{i,i}=\max(\lambda_i,0)$, $i=1,2,\ldots,s$, corresponds to the positive eigenvalues  and $\Lambda_2$, given by $(\Lambda_2)_{i,i}=\max(-\lambda_i,0)$, $i=1,2,\ldots,s$, corresponds to the negative eigenvalues. In this way, we obtain 
\begin{equation}
    U_1\coloneqq (A_kV)\Lambda_1^{1/2}\quad\mathrm{and}\quad U_2\coloneqq (A_kV)\Lambda_2^{1/2}\,.
\end{equation}
Theoretically, it is guaranteed that $M_k=M_{k,0}+ U_1U_1^\top-U_2U_2^\top $ is positive definite \cite{fletcher2013practical} if $s^ky^k>0$ for any $k\in\N$. However, in order to account for numerical rounding errors, we adopt a scaling version:
%in the experiment (Section \ref{sec:experiment}), the smallest eigenvalue of $M_k$ may not be strictly positive due to computational error. We adopt a scaling version:
\begin{equation}\label{eq:metric-scalling}
    M_k=M_{k,0}+ \gamma_1U_1U_1^\top - \gamma_2U_2U_2^\top \,,
\end{equation}
where we set $\gamma_1=1$, $\gamma_2 = 0.99$ in practice. There is an easy way to make sure that Assumption~\ref{assumption1} is satisfied by setting $\gamma_1 = \frac{\eta_k}{\norm[]{U_1}^2}$ and  $\gamma_2 = \frac{\eta_k}{\norm[]{U_2}^2}$. 
\todo[]{The discussion that Assumption 1 is satisfied lacks important details. For instance, it is not clear why $M_{k+1} \leq (1+ \eta_k) M_k$ is satisfied. Further, details on $\eta_k$ are missing. Is this sequence arbitrary in $\ell_1^+$? There is also no discussion on the condition $M_k \in S_\alpha(X)$ which appears to be crucial.}

==> experiment.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% New Section %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Numerical Experiment} \label{sec:experiment}
\todoSW[]{How is the other parameters chosen. What has been done to make sure that the hyperparameters don't pollute the conclusions}
We apply our proposed algorithm for solving a challenging non-smooth image deblurring problem under a Poisson noise assumption \cite{vardi1985statistical}. Given the observation $b\in \R^{n_x\times n_y}$ as $n_x\times n_y$-sized image, the task is the following popular problem:
\begin{equation} \label{eq:deblurring-experiment-primal}
    %\min_{x\in \mathbb{R}_+^{n_x \times n_y}} \underbrace{D_{KL}(b,Ax)}_{h(x)} +\underbrace{\mu \norm[2,1]{\mathcal{D}x}}_{f(x)} \,,
    \min_{x\in \mathbb{R}_+^{n_x \times n_y}} D_{KL}(b,Ax) + \gamma \norm[2,1]{\mathcal{D}x} \,,
\end{equation}
which involves the Kullback--Leibler divergence as data fidelity measure 
$%\[
h(x)\coloneqq D_{\mathrm{KL}}(b,Ax)\coloneqq\sum_{i,j} (Ax)_{i,j}-b_{i,j} \log((Ax)_{i,j})
$ %\]
with respect to the blurred reconstruction $Ax$ with known blur operator and a discrete total variation regularization term $f(x)=\gamma \norm[2,1]{\mathcal{D}x}$ that is steered by a weight $\gamma>0$ where $\mathcal{D}$ implements discrete spatial finite differences. 
We recast \eqref{eq:deblurring-experiment-primal} into the saddle point problem:
\begin{equation}\label{eq:num-exp-deblurr-poisson-saddle}
    %\min_{x\in \mathbb{R}^{n_x \times n_y}} \max_{y\in\R^{2\times n_x\times n_y}}
    %\scal{\mathcal Dx}{y}+ \underbrace{\delta_{\mathbb{R}_+^{n_x \times n_y}}(x)}_{g(x)}+ \underbrace{D_{KL}(b,Ax)}_{h(x)} -\underbrace{\delta_{\norm[2,\infty]{\cdot}\leq \mu} (y)}_{f^*(y)}
    \min_{x\in \mathbb{R}^{n_x \times n_y}} \max_{y\in\R^{2\times n_x\times n_y}}
    \scal{\mathcal Dx}{y}+ \delta_{\mathbb{R}_+^{n_x \times n_y}}(x)+ D_{KL}(b,Ax) -\delta_{\norm[2,\infty]{\cdot}\leq \gamma} (y)
\end{equation}
and set $g(x):=\delta_{\mathbb{R}_+^{n_x \times n_y}}(x)$ and $K=\mathcal D$ in \eqref{eq:saddle-point-problem}. 
Figure~\ref{fig:BFGSmemory} compares several methods including PDHG with fixed stepsize (\texttt{PDHG}), PDHG with line search (\texttt{PDAL}), PDHG with fixed stepsize and variable metric (\texttt{VarPDHG}), PDHG with variable metric and line search (\texttt{VarPDAL}). The variable metric is generated by the limited memory BFGS method in Section~\ref{sec:bfgs-sr1-metric}. Figure~\ref{fig:BFGSmemory} shows the primal gap where the optimal primal value was computed for 10000 iterations by running \texttt{PDHG}. For the update of the variable metric \eqref{eq:metric-scalling}, we set $\gamma_1 =1.0$ and $\gamma_2 =0.99$. However, the Assumption~\ref{assumption1} is not satisfied since it is not guaranteed by the construction of the metric that there is a sequence $(\eta_k)_k\in\ell^1_+(\N)$ such that $M_{k+1}\preceq (1+\eta_k)M_k$. Fortunately, we still observe convergence of PDHG with this variable metric. Figure~\ref{fig:BFGSmemory} shows that a variable metric (\texttt{VarPDHG}) improves the convergence vs only using line search. However, our algorithm \texttt{VarPDAL} that combines both features is even faster, with the best performance when $m=9$. 
% \subsection{The key problem of failure cases}
% In the following experiment, we always set $M_{k,0}=id$. By following the same step as \cite{kanzow2022efficient} in order to get metric in the form of (\ref{metric}), we notice that at some iterates, $M_k$ is not positive definite which results in the crash or weird behavior of the algorithms. So I scaled $U_2$ by $\gamma U_2$ to make sure $M_k = M_{k,0} + U_1U_2^\top  -\gamma^2U_2U_2^\top $ positive definite. Then we obtain the figure \ref{fig:BFGSmemory}.
% \begin{figure}[H]
%     \centering
%     \tikz{
%         \node (A)   {\includegraphics[width=0.53\linewidth]{figure/deblurring image under Poisson noise BFGSloglog.pdf}};
%     %\node[below=0.5mm of A, text width=0.3\linewidth, align=center] (a) {Noisy image };
%          \node[right=-1cm of A] (B) {\includegraphics[width=0.53\linewidth]{figure/deblurring image under Poisson noise BFGS(time).pdf}};
%   %\node[below = 0.5 mm of B, text width=0.3\linewidth, align=center] (b) {Recovered by PDHG line search };
%     }
%     \caption{\label{fig:BFGSmemory}We compare line search PDHG and limited memory variable metric line search PDHG methods. $m$ refers to the number of steps memorized. }
% \end{figure}

% \begin{figure}[th]
%     \centering
%     \tikz{
%         \node (A)   {\includegraphics[width=0.53\linewidth]{figure/deblurring image under Poisson noise BFGS(New).pdf}};
%     %\node[below=0.5mm of A, text width=0.3\linewidth, align=center] (a) {Noisy image };
%          \node[right=-1cm of A] (B) {\includegraphics[width=0.53\linewidth]{figure/deblurring image under Poisson noise BFGS(time)(New).pdf}};
%          \node[below= 0.5 cm of A](C){
%          \includegraphics[width=0.53\linewidth]{figure/deblurring image under Poisson noise BFGS New.pdf}
%          }
%          \node[right = -1cm of C](D){
%          \includegraphics[width=0.53\linewidth]{figure/deblurring image under Poisson noise BFGS(time) New.pdf}
%          }
%   %\node[below = 0.5 mm of B, text width=0.3\linewidth, align=center] (b) {Recovered by PDHG line search };
  
%     }
    
   
%     \caption{\label{fig:BFGSmemory}Performance evaluation for the experiment in \eqref{eq:num-exp-deblurr-poisson-saddle}. Algorithms are described in the text. Our algorithms, which combine a quasi-Newton variable metric with line search, outperform all other algorithms (that either use a variable metric \texttt{VarPDHG} or line search \texttt{PDAL}; or none of the two \texttt{PDHG}).}
% \end{figure}

As a second experiment to test out accelerated version \todoSW[]{Why is there not comparison to an accelerated PDHG;Also, PDAL appears to be the best performing method}, we consider $A=\opid$ and a constraint set $\mathcal{C}\coloneqq \{x\vert x_{ij}\in [\epsilon,255]\}$ since the grey value of each pixel should be less than 255 and be positive; We set $\epsilon=0.1$.
In this case $D_{KL}(b,x)$ restricted on $\mathcal{C}$ is a strongly convex function. We apply the accelerated version of Algorithm \ref{Alg:QN-PDHG-line} in Theorem~\ref{thm:conv-rate-strong-convex}, and we use the notation \texttt{VarAPDAL}. Similary, \texttt{APDAL} denotes the accelerated version of \texttt{PDAL}. The dashed line in \ref{fig:BFGSmemory-g-StrongConvex} corresponds to $O(1/N^2)$. We can observe that \texttt{VarPDAL}, \texttt{APDAL} can converge faster than $O(1/N^2)$ as predicted by the convergence theorem.

% \begin{figure}[th]
%     \centering
%     \tikz{
%         \node (A)   {\includegraphics[width=0.53\linewidth]{figure/deblurring image under Poisson noise BFGS acc.pdf}};
%     %\node[below=0.5mm of A, text width=0.3\linewidth, align=center] (a) {Noisy image };
%          \node[right=-1cm of A] (B) {\includegraphics[width=0.53\linewidth]{figure/deblurring image under Poisson noise BFGS acc(time).pdf}};
%   \node[below = 0.5 mm of B, text width=0.3\linewidth, align=center] (b) {Recovered by PDHG line search };
    
%     \node[below= 1cm of A](C){\includegraphics[width=0.53\linewidth]{figure/deblurring image under Poisson noise BFGS acc Second.pdf}};
%     \node[right= -1cm of C](D){\includegraphics[width=0.53\linewidth]{figure/deblurring image under Poisson noise BFGS acc(time) Second.pdf}};
%     }
%     \caption{\label{fig:BFGSmemory-g-StrongConvex}Performance evaluation for the experiment for a strongly convex case. This figure reflects that our algorithms can retrieve $O(1/N^2)$ convergence rate as \texttt{PDAL}, which is theoretically guaranteed by theorem \ref{thm:conv-rate-strong-convex}.}
% \end{figure}


\todoSW[]{Reviewer#1:the authors should make clearer plots in Fig1 and 2. ! comparing the performance of VarPDAL against the memory and then only considering the best one in the comparison with PDHG, PDAL, VarPDHG}


\section{Conclusion}

In this paper, we introduced a line search variant of a recently introduced quasi-Newton primal-dual algorithm. In contrast to related work, the employed quasi-Newton metric is of type ``identity $\pm$ low rank'', which captures significantly more second order information than a commonly used diagonal metric. We equally care for both, theoretical convergence guarantees including convergence rates as well as efficient practical implementation. The additional line search procedure usually leads to larger steps at a computational cost that pays off, which is confirmed by our numerical experiments. 
